Compliant finray-effect gripper for high-speed robotic assembly of electrical components

Fine assembly tasks such as electrical connector insertion have tight tolerances and sensitive components, limiting the speed and robustness of robot assembly, even when using vision, tactile, or force sensors. Connector insertion is a common industrial task, requiring horizontal alignment errors to be compensated with minimal force, then sufficient force to be brought in the insertion direction. The ability to handle a variety of objects, achieve high-speeds, and handle a wide range in object position variation are also desired. Soft grippers can allow the gripping of parts with variation in surface geometry, but often focus on gripping alone and may not be able to bring the assembly forces required. To achieve high-speed connector insertion, this paper proposes monolithic fingers with structured compliance and form-closure features. A finray-effect gripper is adapted to realize structured (i.e. directional) stiffness that allows high-speed mechanical search, self-alignment in insertion, and sufficient assembly force. The design of the finray ribs and fingertips are investigated, with a final design allowing plug insertion with a tolerance window of up to 7.5 mm at high speed.

==> scraps.tex <==

% Additionally, the varying sizes of the pins and holes and the small tolerances between plug and socket prevent a fast assembly and search strategy. The tolerances between plug and socket are type-specific regarding the geometry of the plug and socket and the number and geometry of pins. Further, the material of the socket, e.g. if manufactured from flexible materials, increases the complexity of the process. An unknown pose of the grasped cable inside the grip is also a major contribution to the complexity \cite{li2014localization}. Angular displacements can be tolerated to a certain degree, exceeding this results in a failed assembly \cite{Yumbla.2019}. The final connection or mating phase can be viewed in detail in \cite{FeiChen.2013} using a cable connection process on a PCB (printed circuit board), where the contact environment is described as a mass-spring-damper model. 

% The assembly of connectors can be divided into three steps: grasping from a magazine, search and insert. For an optimal approach, the position of the part to be gripped and the target has to be known as precisely as possible. Before connecting the ends, a parallel alignment needs to be achieved during the searching process, transitioning to the connection process. Complexity of the search and insert process increases due to the tolerances between plug and socket. Additionally, the varying sizes of the pins and holes and the small tolerances between plug and socket prevent a fast assembly and search strategy. The tolerances between plug and socket are type-specific regarding the geometry of the plug and socket and the number and geometry of pins. Further, the material of the socket, e.g. if manufactured from flexible materials, increases the complexity of the process. An unknown pose of the grasped cable inside the grip is also a major contribution to the complexity \cite{li2014localization}. Angular displacements can be tolerated to a certain degree, exceeding this results in a failed assembly \cite{Yumbla.2019}. The final connection or mating phase can be viewed in detail in \cite{FeiChen.2013} using a cable connection process on a PCB (printed circuit board), where the contact environment is described as a mass-spring-damper model. 

% Grasping or gripping a part is defined by \cite{birglen2007underactuated} as the prevention of motion of an object, manipulating is understood as the control of the pose of an object. When the stiffness of a gripper is considered, motion is not fully prevented but there is a finite compliance or impedance, which may vary in different directions.


% Since grippers with directionally independent, unstructured compliance in the fingertips, pneumatic grippers and the current compensation mechanisms using an RCC in the flange, have proven to be insufficient for the tasks, passive, structural compliance is instead implemented and investigated. 

% Since grippers with directionally independent, unstructured compliance in the fingertips in Sec. \ref{sec:unstructuredcomp}, pneumatic grippers from Sec. \ref{sec:pneumaticgrip} and the current compensation mechanism from Sec. \ref{sec:flange}, have proven to be insufficient for the tasks, passive, structural compliance is instead implemented and investigated. Passive compliance is referred to as the intrinsic mechanical structural compliance of the gripper \cite{wang1998passive}. 

% The possibility to determine the stiffness or respective, the compliance matrix is also investigated later in Sec. \ref{sec:stiffnes_matrix}. The compliance of a reference point of the endeffector can be described by using a 6x6 compliance matrix, where torques and forces about the reference point result in combined translational and rotational displacement \cite{wang1998passive}. 



% The contribution of this work is the development and investigation of a novel, additively manufactured, monolithic finger design for gripping and assembly of electrical components. For this, a novel gripper design is presented using passive compliance to compensate misalignment in the electrical assembly including the assembly of plugs and sockets and clamping of cables. To the author's best knowledge, there is currently no compliance used in electric assembly for high-speed assembly tasks to compensate misalignment. 
% Other than existing compliance in grippers, compliance here is understood in structures achieving significantly different stiffness values in one or more predefined directions. Here, a high stiffness value is desired in the mounting direction to overcome the assembly forces and to ensure a stable insertion. However, significantly lower values are needed in the direction in which misalignment occurred to achieve compensation. 
% An additional objective of the fingers is to achieve generalization over various cable types and over different assembly tasks.
% Sec. \ref{sec:stateota} attends to give a review of current solutions in the electrical assembly. Sec. \ref{sec:intro_tactsens} discusses the opportunity to introduce tactile sensing with two different working principles in the manipulation task. As this thesis describes another approach to compliance, an overview of the current understanding of compliance is given in Sec. \ref{sec:rel_work}. Afterwards, the requirements and constraints for varying aspects in the electrical assembly are discussed in Sec. \ref{sec:reqconst}. A test environment for later experiments is designed and discussed in Sec. \ref{sec:testenv}. The search strategies used are described in Sec. \ref{sec:searchstrategies}. The varying approaches to compliance in this work and the own understanding of compliance are presented in Sec. \ref{sec:compliance}, which are used to identify the optimal type of compliance. Afterwards, the various designs are iteratively determined and discussed regarding their advantages and disadvantages in Sec. \ref{sec:design}. Failures and problems with the design of the fingers, the connectors, the manufacturing process and the assembly process are discussed in Sec. \ref{sec:failprobs}. After obtaining an optimal design, the mechanical attributes, for example the stiffness of a single finger, the stiffness of preloaded, grasping fingers, the maximum tolerable force and the linked maximum deflection is determined experimentally in Sec. \ref{sec:mech_attr}. Afterwards, in Sec. \ref{sec:FEA_Analytical}, FEA and an analytical model are discussed to determine the mechanical attributes via another approach. The possibility to determine the stiffness or the compliance is also investigated in Sec. \ref{sec:stiffnes_matrix}. 
 
% Applications to evaluate the performance of the finger designs are presented in Sec. \ref{sec:applications}, where the \textit{UR}'s program for assembly is presented in Sec. \ref{sec:ur_program}. The presented applications are the repeatability experiment in Sec. \ref{sec:repeatability_magazine}, the robustness experiments in Sec. \ref{sec:robustness_exp}, to determine the tolerable ranges and limits, and the assembly of clamp connections in Sec. \ref{sec:clamping}. Based on the gathered data from the applications and the mechanical attributes, the optimal finger design is discussed in Sec. \ref{sec:finaldesign}.  

%Compliance in this work is understood as structures achieving significantly different stiffness values in one or more predefined directions. Here, a high stiffness value is desired in the mounting direction, however significantly lower values are needed in the direction in which misalignment occurred to achieve compensation. 
